Sparse Subspace Decomposition for Millimeter Wave MIMO Channel Estimation

Millimeter wave multiple-input multiple-output (MIMO) communication systems must operate over sparse wireless links and will require large antenna arrays to provide high throughput. To achieve sufficient array gains, these systems must learn and adapt to the channel state conditions. However, conventional MIMO channel estimation can not be directly extended to millimeter wave due to the constraints on cost-effective millimeter wave operation imposed on the number of available RF chains. Sparse subspace scanning techniques that search for the best subspace sample from the sounded subspace samples have been investigated for channel estimation.However, the performance of these techniques starts to deteriorate as the array size grows, especially for the hybrid precoding architecture. The millimeter wave channel estimation challenge still remains and should be properly addressed before the system can be deployed and used to its full potential. In this work, we propose a sparse subspace decomposition (SSD) technique for sparse millimeter wave MIMO channel estimation. We formulate the channel estimation as an optimization problem that minimizes the subspace distance from the received subspace samples. Alternating optimization techniques are devised to tractably handle the non-convex problem. Numerical simulations demonstrate that the proposed method outperforms other existing techniques with remarkably low overhead.

==> IEEEabrv <==
IEEEabrv.bib V1.13 (2008/09/30) Copyright (c) 2002-2008 by Michael
Shell See: http://www.michaelshell.org/ for current contact
information.

BibTeX bibliography string definitions of the ABBREVIATED titles
of IEEE journals and magazines and online publications.

This file is designed for bibliography styles that require
abbreviated titles and is not for use in bibliographies that
require full-length titles.

Support sites: http://www.michaelshell.org/tex/ieeetran/
http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/
and/or http://www.ieee.org/

Special thanks to Laura Hyslop and ken Rawson of IEEE for their
help in obtaining the information needed to compile this file.
Also, Volker Kuhlmann and Moritz Borgmann kindly provided some
corrections and additions.

*************************************************************************
Legal Notice: This code is offered as-is without any warranty
either expressed or implied; without even the implied warranty of
MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE! User assumes
all risk. In no event shall IEEE or any contributor to this code
be liable for any damages or losses, including, but not limited
to, incidental, consequential, or any other damages, resulting
from the use or misuse of any information contained here.

All comments are the opinions of their respective authors and are
not necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License
(LPPL) ( http://www.latex-project.org/ ) version 1.3, and may be
freely used, distributed and modified. A copy of the LPPL, version
1.3, is included in the base LaTeX documentation of all
distributions of LaTeX released 2003/12/01 or later. Retain all
contribution notices and credits. ** Modified files should be
clearly indicated as such, including  ** ** renaming them and
changing author support contact information. **

File list of work: IEEEabrv.bib, IEEEfull.bib, IEEEexample.bib,
                   IEEEtran.bst, IEEEtranS.bst, IEEEtranSA.bst,
                   IEEEtranN.bst, IEEEtranSN.bst, IEEEtran_bst_HOWTO.pdf
*************************************************************************


USAGE:

\bibliographystyle{mybstfile}
\bibliography{IEEEabrv,mybibfile}

where the IEEE titles in the .bib database entries use the strings
defined here. e.g.,


   journal = IEEE_J_AC,


to yield "{IEEE} Trans. Automat. Contr."


IEEE uses abbreviated journal titles in their bibliographies -
this file is suitable for work that is to be submitted to the
IEEE.


For work that requires full-length titles, you should use the full
titles provided in the companion file, IEEEfull.bib.


** NOTES **

 1. Journals have been grouped according to subject in order to make it
    easier to locate and extract the definitions for related journals -
    as most works use references that are confined to a single topic.
    Magazines are listed in straight alphabetical order.

 2. String names are closely based on IEEE's own internal acronyms.

 3. Abbreviations follow IEEE's style.

 4. Older, out-of-print IEEE titles are included (but not including titles
    dating prior to IEEE's formation from the IRE and AIEE in 1963).

 5. The following string definitions have been disabled because their
    abbreviations have not yet been verified:

    STRING{IEEE_J_LT         = "{IEEE} Trans. Learning Technol."}
    STRING{IEEE_J_NSM        = "{IEEE} Trans. Netw. Service Manag."}
    STRING{IEEE_J_SC         = "{IEEE} Trans. Services Comput."}
    STRING{IEEE_J_STARS      = "{IEEE} J. Sel. Topics Appl. Earth Observations Remote Sens."}


    If you know what the proper abbreviation is for a string above,
    email me and I will correct them in the next release.





IEEE Journals



aerospace and military @STRING{IEEE_J_AES        = "{IEEE} Trans.
Aerosp. Electron. Syst."} @STRING{IEEE_J_ANE        = "{IEEE}
Trans. Aerosp. Navig. Electron."} @STRING{IEEE_J_ANNE       =
"{IEEE} Trans. Aeronaut. Navig. Electron."} @STRING{IEEE_J_AS
= "{IEEE} Trans. Aerosp."} @STRING{IEEE_J_AIRE       = "{IEEE}
Trans. Airborne Electron."} @STRING{IEEE_J_MIL        = "{IEEE}
Trans. Mil. Electron."}



autos, transportation and vehicles (non-aerospace)
@STRING{IEEE_J_ITS        = "{IEEE} Trans. Intell. Transp. Syst."}
@STRING{IEEE_J_VT         = "{IEEE} Trans. Veh. Technol."}
@STRING{IEEE_J_VC         = "{IEEE} Trans. Veh. Commun."}



circuits, signals, systems, audio and controls @STRING{IEEE_J_SPL
= "{IEEE} Signal Process. Lett."} @STRING{IEEE_J_ASSP       =
"{IEEE} Trans. Acoust., Speech, Signal Process."}
@STRING{IEEE_J_AU         = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA       = "{IEEE} Trans. Audio Electroacoust."}
@STRING{IEEE_J_AC         = "{IEEE} Trans. Autom. Control"}
@STRING{IEEE_J_CAS        = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT      = "{IEEE} Trans. Circuits Syst. Video
Technol."} @STRING{IEEE_J_CASI       = "{IEEE} Trans. Circuits
Syst. {I}"} @STRING{IEEE_J_CASII      = "{IEEE} Trans. Circuits
Syst. {II}"} in 2004 CASI and CASII renamed part title to CASI_RP
and CASII_EB, respectively. @STRING{IEEE_J_CASI_RP    = "{IEEE}
Trans. Circuits Syst. {I}"} @STRING{IEEE_J_CASII_EB   = "{IEEE}
Trans. Circuits Syst. {II}"} @STRING{IEEE_J_CT         = "{IEEE}
Trans. Circuit Theory"} @STRING{IEEE_J_CST        = "{IEEE} Trans.
Control Syst. Technol."} @STRING{IEEE_J_SP         = "{IEEE}
Trans. Signal Process."} @STRING{IEEE_J_SU         = "{IEEE}
Trans. Sonics Ultrason."} @STRING{IEEE_J_SAP        = "{IEEE}
Trans. Speech Audio Process."} @STRING{IEEE_J_STSP       = "{IEEE}
J. Sel. Topics Signal Process."} @STRING{IEEE_J_SYST       =
"{IEEE} Syst. J."} @STRING{IEEE_J_UE         = "{IEEE} Trans.
Ultrason. Eng."} @STRING{IEEE_J_UFFC       = "{IEEE} Trans.
Ultrason., Ferroelectr., Freq. Control"}



communications @STRING{IEEE_J_COML       = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC       = "{IEEE} J. Sel. Areas Commun."}
@STRING{IEEE_J_COM        = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT       = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM       = "{IEEE} Trans. Wireless Commun."}



components, packaging and manufacturing @STRING{IEEE_J_ADVP
= "{IEEE} Trans. Adv. Packag."} @STRING{IEEE_J_CHMT       =
"{IEEE} Trans. Compon., Hybrids, Manuf. Technol."}
@STRING{IEEE_J_CPMTA      = "{IEEE} Trans. Compon., Packag.,
Manuf. Technol. {A}"} @STRING{IEEE_J_CPMTB      = "{IEEE} Trans.
Compon., Packag., Manuf. Technol. {B}"} @STRING{IEEE_J_CPMTC
= "{IEEE} Trans. Compon., Packag., Manuf. Technol. {C}"}
@STRING{IEEE_J_CAPT       = "{IEEE} Trans. Compon. Packag.
Technol."} @STRING{IEEE_J_CAPTS      = "{IEEE} Trans. Compon.
Packag. Technol."} @STRING{IEEE_J_CPART      = "{IEEE} Trans.
Compon. Parts"} @STRING{IEEE_J_EPM        = "{IEEE} Trans.
Electron. Packag. Manuf."} @STRING{IEEE_J_MFT        = "{IEEE}
Trans. Manuf. Technol."} @STRING{IEEE_J_PHP        = "{IEEE}
Trans. Parts, Hybrids, Packag."} @STRING{IEEE_J_PMP        =
"{IEEE} Trans. Parts, Mater., Packag."}



CAD @STRING{IEEE_J_TCAD       = "{IEEE} J. Technol. Comput. Aided
Design"} @STRING{IEEE_J_CAD        = "{IEEE} Trans. Comput.-Aided
Design Integr. Circuits Syst."}



coding, data, information, knowledge @STRING{IEEE_J_IT         =
"{IEEE} Trans. Inf. Theory"} @STRING{IEEE_J_KDE        = "{IEEE}
Trans. Knowl. Data Eng."}



computers, computation, networking and software @STRING{IEEE_J_C
= "{IEEE} Trans. Comput."} @STRING{IEEE_J_CAL        = "{IEEE}
Comput. Archit. Lett."} @STRING{IEEE_J_DSC        = "{IEEE} Trans.
Dependable Secure Comput."} @STRING{IEEE_J_ECOMP      = "{IEEE}
Trans. Electron. Comput."} @STRING{IEEE_J_EVC        = "{IEEE}
Trans. Evol. Comput."} @STRING{IEEE_J_FUZZ       = "{IEEE} Trans.
Fuzzy Syst."} @STRING{IEEE_J_IFS        = "{IEEE} Trans. Inf.
Forensics Security"} @STRING{IEEE_J_MC         = "{IEEE} Trans.
Mobile Comput."} @STRING{IEEE_J_NET        = "{IEEE/ACM} Trans.
Netw."} @STRING{IEEE_J_NN         = "{IEEE} Trans. Neural Netw."}
disabled until abbreviation verified STRING{IEEE_J_NSM        =
"{IEEE} Trans. Netw. Service Manag."} @STRING{IEEE_J_PDS        =
"{IEEE} Trans. Parallel Distrib. Syst."} disabled until
abbreviation verified STRING{IEEE_J_SC         = "{IEEE} Trans.
Services Comput."} @STRING{IEEE_J_SE         = "{IEEE} Trans.
Softw. Eng."}



computer graphics, imaging, and multimedia @STRING{IEEE_J_JDT
= "{IEEE/OSA} J. Display Technol."} @STRING{IEEE_J_IP         =
"{IEEE} Trans. Image Process."} @STRING{IEEE_J_MM         =
"{IEEE} Trans. Multimedia"} @STRING{IEEE_J_VCG        = "{IEEE}
Trans. Vis. Comput. Graphics"}



cybernetics, ergonomics, robots, man-machine, and automation
@STRING{IEEE_J_ASE        = "{IEEE} Trans. Autom. Sci. Eng."}
@STRING{IEEE_J_JRA        = "{IEEE} J. Robot. Autom."}
@STRING{IEEE_J_H          = "{IEEE} Trans. Haptics"}
@STRING{IEEE_J_HFE        = "{IEEE} Trans. Hum. Factors
Electron."} @STRING{IEEE_J_MMS        = "{IEEE} Trans. Man-Mach.
Syst."} @STRING{IEEE_J_PAMI       = "{IEEE} Trans. Pattern Anal.
Mach. Intell."} in 1989 JRA became RA in August 2004, RA split
into ASE and RO @STRING{IEEE_J_RA         = "{IEEE} Trans. Robot.
Autom."} @STRING{IEEE_J_RO         = "{IEEE} Trans. Robot."}
@STRING{IEEE_J_SMC        = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA       = "{IEEE} Trans. Syst., Man, Cybern.
{A}"} @STRING{IEEE_J_SMCB       = "{IEEE} Trans. Syst., Man,
Cybern. {B}"} @STRING{IEEE_J_SMCC       = "{IEEE} Trans. Syst.,
Man, Cybern. {C}"} @STRING{IEEE_J_SSC        = "{IEEE} Trans.
Syst. Sci. Cybern."}



earth, wind, fire and water @STRING{IEEE_J_GE         = "{IEEE}
Trans. Geosci. Electron."} @STRING{IEEE_J_GRS        = "{IEEE}
Trans. Geosci. Remote Sens."} @STRING{IEEE_J_GRSL       = "{IEEE}
Geosci. Remote Sens. Lett."} @STRING{IEEE_J_OE         = "{IEEE}
J. Ocean. Eng."} disabled until abbreviation verified
STRING{IEEE_J_STARS      = "{IEEE} J. Sel. Topics Appl. Earth
Observations Remote Sens."}


education, engineering, history, IEEE, professional
@STRING{IEEE_J_CJECE      = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC       = "Proc. {IEEE}"} @STRING{IEEE_J_EDU
= "{IEEE} Trans. Educ."} @STRING{IEEE_J_EM         = "{IEEE}
Trans. Eng. Manag."} @STRING{IEEE_J_EWS        = "{IEEE} Trans.
Eng. Writing Speech"} disabled until abbreviation verified
STRING{IEEE_J_LT         = "{IEEE} Trans. Learning Technol."}
@STRING{IEEE_J_PC         = "{IEEE} Trans. Prof. Commun."}



electromagnetics, antennas, EMI, magnetics and microwave
@STRING{IEEE_J_AWPL       = "{IEEE} Antennas Wireless Propag.
Lett."} @STRING{IEEE_J_MGWL       = "{IEEE} Microw. Guided Wave
Lett."} IEEE seems to want "Compon." here, not "Comp."
@STRING{IEEE_J_MWCL       = "{IEEE} Microw. Wireless Compon.
Lett."} @STRING{IEEE_J_AP         = "{IEEE} Trans. Antennas
Propag."} @STRING{IEEE_J_EMC        = "{IEEE} Trans. Electromagn.
Compat."} @STRING{IEEE_J_MAG        = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT        = "{IEEE} Trans. Microw. Theory Tech."}
@STRING{IEEE_J_RFI        = "{IEEE} Trans. Radio Freq.
Interference"} @STRING{IEEE_J_TJMJ       = "{IEEE} Transl. J.
Magn. Jpn."}



energy and power @STRING{IEEE_J_EC         = "{IEEE} Trans. Energy
Convers."} @STRING{IEEE_J_PEL        = "{IEEE} Power Electron.
Lett."} @STRING{IEEE_J_PWRAS      = "{IEEE} Trans. Power App.
Syst."} @STRING{IEEE_J_PWRD       = "{IEEE} Trans. Power Del."}
@STRING{IEEE_J_PWRE       = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS       = "{IEEE} Trans. Power Syst."}



industrial, commercial and consumer @STRING{IEEE_J_APPIND     =
"{IEEE} Trans. Appl. Ind."} @STRING{IEEE_J_BC         = "{IEEE}
Trans. Broadcast."} @STRING{IEEE_J_BCTV       = "{IEEE} Trans.
Broadcast Television Receivers"} @STRING{IEEE_J_CE         =
"{IEEE} Trans. Consum. Electron."} @STRING{IEEE_J_IE         =
"{IEEE} Trans. Ind. Electron."} @STRING{IEEE_J_IECI       =
"{IEEE} Trans. Ind. Electron. Contr. Instrum."} @STRING{IEEE_J_IA
= "{IEEE} Trans. Ind. Appl."} @STRING{IEEE_J_IGA        = "{IEEE}
Trans. Ind. Gen. Appl."} @STRING{IEEE_J_IINF       = "{IEEE}
Trans. Ind. Informat."} @STRING{IEEE_J_PSE        = "{IEEE} J.
Product Safety Eng."}



instrumentation and measurement @STRING{IEEE_J_IM         =
"{IEEE} Trans. Instrum. Meas."}



insulation and materials @STRING{IEEE_J_JEM        = "{IEEE/TMS}
J. Electron. Mater."} @STRING{IEEE_J_DEI        = "{IEEE} Trans.
Dielectr. Electr. Insul."} @STRING{IEEE_J_EI         = "{IEEE}
Trans. Electr. Insul."}



mechanical @STRING{IEEE_J_MECH       = "{IEEE/ASME} Trans.
Mechatronics"} @STRING{IEEE_J_MEMS       = "J. Microelectromech.
Syst."}



medical and biological @STRING{IEEE_J_BCAS       = "{IEEE} Trans.
Biomed. Circuits Syst."} @STRING{IEEE_J_BME        = "{IEEE}
Trans. Biomed. Eng."} Note: The B-ME journal later dropped the
hyphen and became the BME. @STRING{IEEE_J_B-ME       = "{IEEE}
Trans. Bio-Med. Eng."} @STRING{IEEE_J_BMELC      = "{IEEE} Trans.
Bio-Med. Electron."} @STRING{IEEE_J_CBB        = "{IEEE/ACM}
Trans. Comput. Biol. Bioinformatics"} @STRING{IEEE_J_ITBM       =
"{IEEE} Trans. Inf. Technol. Biomed."} @STRING{IEEE_J_ME         =
"{IEEE} Trans. Med. Electron."} @STRING{IEEE_J_MI         =
"{IEEE} Trans. Med. Imag."} @STRING{IEEE_J_NB         = "{IEEE}
Trans. Nanobiosci."} @STRING{IEEE_J_NSRE       = "{IEEE} Trans.
Neural Syst. Rehabil. Eng."} @STRING{IEEE_J_RBME       = "{IEEE}
Rev. Biomed. Eng."} @STRING{IEEE_J_RE         = "{IEEE} Trans.
Rehabil. Eng."}



 optics, lightwave and photonics
@STRING{IEEE_J_PTL        = "{IEEE} Photon. Technol. Lett."}
@STRING{IEEE_J_JLT        = "J. Lightw. Technol."}



physics, electrons, nanotechnology, nuclear and quantum
electronics @STRING{IEEE_J_EDL        = "{IEEE} Electron Device
Lett."} @STRING{IEEE_J_JQE        = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE      = "{IEEE} J. Sel. Topics Quantum
Electron."} @STRING{IEEE_J_ED         = "{IEEE} Trans. Electron
Devices"} @STRING{IEEE_J_NANO       = "{IEEE} Trans.
Nanotechnol."} @STRING{IEEE_J_NS         = "{IEEE} Trans. Nucl.
Sci."} @STRING{IEEE_J_PS         = "{IEEE} Trans. Plasma Sci."}



reliability IEEE seems to want "Mat." here, not "Mater."
@STRING{IEEE_J_DMR        = "{IEEE} Trans. Device Mater. Rel."}
@STRING{IEEE_J_R          = "{IEEE} Trans. Rel."}



semiconductors, superconductors, electrochemical and solid state
@STRING{IEEE_J_ESSL       = "{IEEE/ECS} Electrochem. Solid-State
Lett."} @STRING{IEEE_J_JSSC       = "{IEEE} J. Solid-State
Circuits"} @STRING{IEEE_J_ASC        = "{IEEE} Trans. Appl.
Supercond."} @STRING{IEEE_J_SM         = "{IEEE} Trans. Semicond.
Manuf."}



sensors @STRING{IEEE_J_SENSOR     = "{IEEE} Sensors J."}



VLSI @STRING{IEEE_J_VLSI       = "{IEEE} Trans. {VLSI} Syst."}






IEEE Magazines



@STRING{IEEE_M_AES        = "{IEEE} Aerosp. Electron. Syst. Mag."}
@STRING{IEEE_M_HIST       = "{IEEE} Ann. Hist. Comput."}
@STRING{IEEE_M_AP         = "{IEEE} Antennas Propag. Mag."}
@STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CD         = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS        = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM        = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC     = "{IEEE} Commun. Soc. Mag."}
@STRING{IEEE_M_CIM        = "{IEEE} Comput. Intell. Mag."} CSEM
changed to CSE in 1999 @STRING{IEEE_M_CSE        = "{IEEE} Comput.
Sci. Eng."} @STRING{IEEE_M_CSEM       = "{IEEE} Comput. Sci. Eng.
Mag."} @STRING{IEEE_M_C          = "{IEEE} Computer"}
@STRING{IEEE_M_CAP        = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA        = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS         = "{IEEE} Control Syst. Mag."}
@STRING{IEEE_M_DTC        = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_M_EI         = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_ETR        = "{IEEE} ElectroTechnol. Rev."}
@STRING{IEEE_M_EMB        = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EMR        = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EXP        = "{IEEE} Expert"} @STRING{IEEE_M_IA
= "{IEEE} Ind. Appl. Mag."} @STRING{IEEE_M_IE         = "{IEEE}
Ind. Electron. Mag."} @STRING{IEEE_M_IM         = "{IEEE} Instrum.
Meas. Mag."} @STRING{IEEE_M_IS         = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_ITS        = "{IEEE} Intell. Transp. Syst. Mag."}
@STRING{IEEE_M_IC         = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP        = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO      = "{IEEE} Micro"} @STRING{IEEE_M_MW
= "{IEEE} Microw. Mag."} @STRING{IEEE_M_MM         = "{IEEE}
Multimedia"} @STRING{IEEE_M_NANO       = "{IEEE} Nanotechnol.
Mag."} @STRING{IEEE_M_NET        = "{IEEE} Netw."} IEEE's
editorial manual lists "Pers. Commun.", but "Personal Commun.
Mag." seems to be what is used in the journals @STRING{IEEE_M_PCOM
= "{IEEE} Personal Commun. Mag."} @STRING{IEEE_M_POT        =
"{IEEE} Potentials"} CAP and PER merged to form PE in 2003
@STRING{IEEE_M_PE         = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER        = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_PVC        = "{IEEE} Pervasive Comput."}
@STRING{IEEE_M_RA         = "{IEEE} Robot. Autom. Mag."}
@STRING{IEEE_M_SAP        = "{IEEE} Security Privacy"}
@STRING{IEEE_M_SP         = "{IEEE} Signal Process. Mag."}
@STRING{IEEE_M_S          = "{IEEE} Softw."} @STRING{IEEE_M_SPECT
= "{IEEE} Spectr."} @STRING{IEEE_M_TS         = "{IEEE} Technol.
Soc. Mag."} @STRING{IEEE_M_VT         = "{IEEE} Veh. Technol.
Mag."} @STRING{IEEE_M_WC         = "{IEEE} Wireless Commun. Mag."}
@STRING{IEEE_M_TODAY      = "Today's Engineer"}






IEEE Online Publications



@STRING{IEEE_O_CSTO        = "{IEEE} Commun. Surveys Tuts."}
@STRING{IEEE_O_DSO         = "{IEEE} Distrib. Syst. Online"}





-- EOF


==> ctextemp_mydefinitions.tex <==
\def\CTeXPreproc{Created by ctex v0.2.13, don't edit!}% Calligraphic uppercase
\def\cA{{\mathcal{A}}} \def\cB{{\mathcal{B}}} \def\cC{{\mathcal{C}}} \def\cD{{\mathcal{D}}}
\def\cE{{\mathcal{E}}} \def\cF{{\mathcal{F}}} \def\cG{{\mathcal{G}}} \def\cH{{\mathcal{H}}}
\def\cI{{\mathcal{I}}} \def\cJ{{\mathcal{J}}} \def\cK{{\mathcal{K}}} \def\cL{{\mathcal{L}}}
\def\cM{{\mathcal{M}}} \def\cN{{\mathcal{N}}} \def\cO{{\mathcal{O}}} \def\cP{{\mathcal{P}}}
\def\cQ{{\mathcal{Q}}} \def\cR{{\mathcal{R}}} \def\cS{{\mathcal{S}}} \def\cT{{\mathcal{T}}}
\def\cU{{\mathcal{U}}} \def\cV{{\mathcal{V}}} \def\cW{{\mathcal{W}}} \def\cX{{\mathcal{X}}}
\def\cY{{\mathcal{Y}}} \def\cZ{{\mathcal{Z}}}

% Bold lowercase
\def\ba{{\mathbf{a}}} \def\bb{{\mathbf{b}}} \def\bc{{\mathbf{c}}} \def\bd{{\mathbf{d}}} \def\be{{\mathbf{e}}}
\def\bff{{\mathbf{f}}} \def\bg{{\mathbf{g}}} \def\bhh{{\mathbf{h}}} \def\bi{{\mathbf{i}}} \def\bj{{\mathbf{j}}}
\def\bk{{\mathbf{k}}} \def\bl{{\mathbf{l}}} \def\bm{{\mathbf{m}}} \def\bn{{\mathbf{n}}} \def\bo{{\mathbf{o}}}
\def\bp{{\mathbf{p}}} \def\bq{{\mathbf{q}}} \def\br{{\mathbf{r}}} \def\bs{{\mathbf{s}}} \def\bt{{\mathbf{t}}}
\def\bu{{\mathbf{u}}} \def\bv{{\mathbf{v}}} \def\bw{{\mathbf{w}}} \def\bx{{\mathbf{x}}} \def\by{{\mathbf{y}}}
\def\bz{{\mathbf{z}}} \def\bh{\mathbf{h}}

% Bold capital letters
\def\bA{{\mathbf{A}}} \def\bB{{\mathbf{B}}} \def\bC{{\mathbf{C}}} \def\bD{{\mathbf{D}}} \def\bE{{\mathbf{E}}}
\def\bF{{\mathbf{F}}} \def\bG{{\mathbf{G}}} \def\bH{{\mathbf{H}}} \def\bI{{\mathbf{I}}} \def\bJ{{\mathbf{J}}}
\def\bK{{\mathbf{K}}} \def\bL{{\mathbf{L}}} \def\bM{{\mathbf{M}}} \def\bN{{\mathbf{N}}} \def\bO{{\mathbf{O}}}
\def\bP{{\mathbf{P}}} \def\bQ{{\mathbf{Q}}} \def\bR{{\mathbf{R}}} \def\bS{{\mathbf{S}}} \def\bT{{\mathbf{T}}}
\def\bU{{\mathbf{U}}} \def\bV{{\mathbf{V}}} \def\bW{{\mathbf{W}}} \def\bX{{\mathbf{X}}} \def\bY{{\mathbf{Y}}}
\def\bZ{{\mathbf{Z}}}

% Italic bold lowercase
\def\iba{{\pmb{a}}} \def\ibb{{\pmb{b}}} \def\ibc{{\pmb{c}}} \def\ibd{{\pmb{d}}} \def\ibe{{\pmb{e}}}
\def\ibf{{\pmb{f}}} \def\ibg{{\pmb{g}}} \def\ibh{{\pmb{h}}} \def\ibi{{\pmb{i}}} \def\ibj{{\pmb{j}}}
\def\ibk{{\pmb{k}}} \def\ibl{{\pmb{l}}} \def\ibm{{\pmb{m}}} \def\ibn{{\pmb{n}}} \def\ibo{{\pmb{o}}}
\def\ibp{{\pmb{p}}} \def\ibq{{\pmb{q}}} \def\ibr{{\pmb{r}}} \def\ibs{{\pmb{s}}} \def\ibt{{\pmb{t}}}
\def\ibu{{\pmb{u}}} \def\ibv{{\pmb{v}}} \def\ibw{{\pmb{w}}} \def\ibx{{\pmb{x}}} \def\iby{{\pmb{y}}}
\def\ibz{{\pmb{z}}}

% Italic bold capital letters
\def\ibA{{\pmb{A}}} \def\ibB{{\pmb{B}}} \def\ibC{{\pmb{C}}} \def\ibD{{\pmb{D}}} \def\ibE{{\pmb{E}}}
\def\ibF{{\pmb{F}}} \def\ibG{{\pmb{G}}} \def\ibH{{\pmb{H}}} \def\ibI{{\pmb{I}}} \def\ibJ{{\pmb{J}}}
\def\ibK{{\pmb{K}}} \def\ibL{{\pmb{L}}} \def\ibM{{\pmb{M}}} \def\ibN{{\pmb{N}}} \def\ibO{{\pmb{O}}}
\def\ibP{{\pmb{P}}} \def\ibQ{{\pmb{Q}}} \def\ibR{{\pmb{R}}} \def\ibS{{\pmb{S}}} \def\ibT{{\pmb{T}}}
\def\ibU{{\pmb{U}}} \def\ibV{{\pmb{V}}} \def\ibW{{\pmb{W}}} \def\ibX{{\pmb{X}}} \def\ibY{{\pmb{Y}}}
\def\ibZ{{\pmb{Z}}}

% Math
\def\argmin{\mathop{\mathrm{argmin}}}
\def\argmax{\mathop{\mathrm{argmax}}}
\def\det{\mathop{\mathrm{det}}}
\def\arccos{\mathop{\mathrm{arccos\!}}}
\def\e{{\mathrm{e}}}
\def\tr{\mathop{\mathrm{tr}}}
\def\real{\mathop{\mathrm{Re\!}}}
\def\dim{\mathop{\mathrm{dim}}}
\def\vol{{\mathop{vol}}}
\def\Cup{\mathop{\mathrm{{\bigcup}}}}
\def\const{\mathop{\mathrm{Const.}}}
\def\rank{\mathop{\mathrm{rank}}}
\def\span{\mathop{\mathrm{span}}}
\def\vec{\mathop{\mathrm{vec}}}
\def\cov{\mathop{\mathrm{cov}}}
\def\diag{\mathop{\mathrm{diag}}}
\def\intf{\mathop{\mathrm{int}}}
\def\mod{\mathop{\mathrm{mod}}}
\def\bzeros{\mathbf{0}}
\def\red{\mathop{\mathrm{red} }}
\def\var{\mathop{\mathrm{var}}}
\def\mse{\mathop{\mathrm{mse}}}

\renewcommand{\baselinestretch}{1.0}
\def\bss{\vspace{\baselineskip}}

% Symbols
\def\ie{{i.e.}}     \def\d4{\!\!\!\!}     \def\t{\tau}         \def\ep{\epsilon}
\def\Mt{M_t}        \def\Mr{M_r}          \def\gam{\gamma}     \def\al{\alpha}
\def\Del{\Delta}    \def\del{\delta}      \def\Gam{\Gamma}     \def\bark{\bar{k}}
\def\bSig{\mathbf{\Sigma}} \def\bsh{\backslash} \def\bGam{\mathbf{\Gamma}} \def\bLam{\mathbf{\Lambda}}
\def\bPi{\mathbf{\Pi}} \def\bPhi{\mathbf{\Phi}} \def\thet{\theta} \def\bmu{\boldsymbol\mu} \def\lam{\lambda} \def\bthe{\boldsymbol{\theta}}
\def\bal{\boldsymbol{\alpha}} \def\blam{\boldsymbol{\lambda}}

% Math bold capital letters
\def\N{{\mathbb{N}}} \def\Q{{\mathbb{Q}}} \def\R{{\mathbb{R}}} \def\C{{\mathbb{C}}} \def\Z{{\mathbb{Z}}} \def\S{{\mathbb{S}}}
\def\bone{\mathbf{1}}

% Parenthesis
\def\lp{\left(}     \def\rp{\right)}    \def\ls{\left\{}    \def\rs{\right\}}    \def\lS{ \left[ }
\def\rS{ \right] }  \def\la{\left|}     \def\ra{\right|}    \def\lA{\left\|}     \def\rA{\right\|}

% \Bar
\def\barD{\bar{D}}  \def\barm{\bar{m}}  \def\barn{\bar{n}} \def\baral{\bar{\al}} \def\bbZ{\bar{\bZ}}
\def\bbY{\bar{\bY}} \def\bbH{\bar{\bH}} \def\bbx{\bar{\bx}} \def\bbSig{\bar{\bSig}} \def\bbV{\bar{\bV}}
\def\bbU{\bar{\bU}} \def\bbX{\bar{\bX}} \def\bby{\bar{\by}} \def\bbz{\bar{\bz}}
\def\bbP{\bar{\bP}} \def\bbG{\bar{\bG}} \def\bbz{\bar{\bz}} \def\bbN{\bar{\bN}} \def\bbA{\bar{\bA}}
\def\bbB{\bar{\bB}} \def\bbLam{\bar{\bLam}} \def\bbF{\bar{\bF}} \def\bbK{\bar{\bK}} \def\bbO{\bar{\bO}}
\def\barw{\bar{w}}  \def\barx{\bar{x}}  \def\bary{\bar{y}}

% \tilde
\def\tn{\tilde{n}}  \def\tm{\tilde{m}}  \def\tB{\tilde{B}}  \def\tbh{\tilde{\bh}}  \def\tbg{\tilde{\bg}}
\def\tgam{\tilde{\gam}} \def\tbG{\widetilde{\bG}} \def\tbP{\widetilde{\bP}} \def\tbH{\widetilde{\bH}} \def\tbA{\widetilde{\bA}} \def\tbB{\widetilde{\bB}}
\def\tby{\tilde{\by}} \def\tbz{\tilde{\bz}} \def\tal{\tilde{\al}} \def\tbs{\tilde{\bs}} \def\tbff{\tilde{\bff}}
\def\th{\tilde{h}} \def\tN{\tilde{N}} \def\sig{\sigma}  \def\tsig{\tilde{\sigma}} \def\tbx{\tilde{\bx}} \def\tba{\tilde{\ba}} \def\tbn{\tilde{\bn}}

% \hat
\def\hbU{\hat{\bU}} \def\hbH{\hat{\bH}} \def\hbN{\hat{\bN}}  \def\hbB{\widehat{\bB}} \def\hu{\hat{u}} \def\hthe{\hat{\theta}} \def\hA{\hat{A}} \def\hbthe{\hat{\bthe}}
\def\hal{\hat{\alpha}}  \def\hbal{\hat{\bal}} \def\hbs{\hat{\bs}} \def\hbx{\hat{\bx}} \def\hcZ{\widehat{\cZ}} \def\hbhh{\hat{\bhh}} \def\hbv{\hat{\bv}}
\def\hbr{\hat{\br}}

% Operators
\def\mul{\! \times \!}  \def\-{\! - \!}  \def\+{\! + \!}  \def\={\! = \!}  \def\>{\! > \!} \def\nn{\nonumber}

\def\pe{p_{e}}
\def\pebeacon{p_{e,beacon}}
\def\pepoll{p_{e,poll}}
\def\pepull{p_{e,pull}}
\def\pedata{p_{e,data}}
\def\peack{p_{e,ack}}
\def\pedataack{p_{e,data+ack}}
\def\tpoll{t_{poll}}
\def\tsifs{t_{sifs}}
\def\tpifs{t_{pifs}}
\def\tpull{t_{pull}}
\def\tpack{t_{pack}}
\def\tdata{t_{data}}
\def\tack{t_{ack}}
\def\tdataack{t_{data+ack}}
\def\wtU{\widetilde{U}}
\def\wtR{\widetilde{\cR}}
\def\hR{\widehat{\cR}}
\def\Ip{I_+}
\def\tIp{\tilde{I}_+}
\def\tp{\tilde{p}}

\def\tcr{\textcolor{red}}
\def\tcb{\textcolor{blue}}
\def\tb{\textbf}

% \newtheorem
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{claim}{Claim}
\newtheorem{definition}{Definition}

% \newcommand
\newcommand{\bef}{\begin{figure}}
\newcommand{\eef}{\end{figure}}
\newcommand{\beq}{\begin{eqnarray}}
\newcommand{\eeq}{\end{eqnarray}}

\newenvironment{proof}[1][Proof]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{definition}[1][Definition:]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{remark}[1][Remark]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

\newcommand{\qed}{\nobreak \ifvmode \relax \else
\ifdim\lastskip<1.5em \hskip-\lastskip \hskip1.5em plus0em
minus0.5em \fi \nobreak \vrule height0.5em width0.5em
depth0.25em\fi}

